Power Measurement Enabled Channel Autocorrelation Matrix Estimation for IRS-Assisted Wireless Communication

By reconfiguring wireless channels via passive signal reflection, intelligent reflecting surface (IRS) can bring significant performance enhancement for wireless communication systems. However, such performance improvement generally relies on the knowledge of channel state information (CSI) for IRS-involved links. Prior works on IRS CSI acquisition mainly estimate IRS-cascaded channels based on the extra pilot signals received at the users/base station (BS) with time-varying IRS reflections, which, however, needs to modify the existing channel training/estimation protocols of wireless systems. To address this issue, we propose in this paper a new channel estimation scheme for IRS-assisted communication systems based on the received signal power measured at the user terminal, which is practically attainable without the need of changing the current protocol. Due to the lack of signal phase information in measured power, the autocorrelation matrix of the BS-IRS-user cascaded channel is estimated by solving an equivalent rank-minimization problem. To this end, a low-rank-approaching (LRA) algorithm is proposed by employing the fractional programming and alternating optimization techniques. To reduce computational complexity, an approximate LRA (ALRA) algorithm is also developed. Furthermore, these two algorithms are extended to be robust against the receiver noise and quantization error in power measurement. Simulation results are provided to verify the effectiveness of the proposed channel estimation algorithms as well as the IRS passive reflection design based on the estimated channel autocorrelation matrix.

==> utils/complm-ver01.tex <==


\section{Complementary Proof of Lemma~\ref{lemma:dim-defficiency}}\label{complm-sec:lemma1-proof}
    In this section, the detailed proof for the dimension of space $\mathcal{S}_X^{b}(N)$ defined in Appendix~\ref{appendix:lemma-proof-dim-deff} is given to complete the proof of Lemma~\ref{lemma:dim-defficiency}, where it is claimed that $\text{dim}(\mathcal{S}_X^{b}(N)) = \mathcal{D}_{N}^{(b)}$. 
    The function $\mathcal{D}_{N}^{(b)}$ is defined in Lemma~\ref{lemma:dim-defficiency} as
    \begin{equation}\label{def:spanned-spaced-dim}
        \mathcal{D}_{N}^{(b)} = \left\{
            \begin{aligned}
                & \frac{N^2 - N}{2} + 1, ~~~ b = 1 \\
                & N^2 - N + 1, ~~~~ b \ge 2
            \end{aligned}
        \right.
        .
    \end{equation}
    To prove $\text{dim}(\mathcal{S}_X^{b}(N)) = \mathcal{D}_{N}^{(b)}$, we first denote the $N^2$-dimensional hermitian matrices space as $\mathcal{S}_H(N)$ and explicitly define an orthonormal basis for it. 
    Then, we show that $\mathcal{S}_X^{b}(N)$ can be spanned by $\mathcal{D}_{N}^{(b)}$ matrices in the basis~\cite{ref:OLS}. 

        \vspace{-6pt}
        \subsection{Orthonormal Basis of Space $\mathcal{S}_H(N)$}\label{complm-subsec:herm-ortho-basis}
            Consider vector $\boldsymbol{b}_1 = \boldsymbol{1}_{N} / \sqrt{N} \in\mathbb{R}^{N\times 1}$, and denote $\boldsymbol{b}_2, \ldots, \boldsymbol{b}_N$ as the vectors that form an orthonormal basis along with $\boldsymbol{b}_1$ for the $N$-dimensional real vector space $\mathbb{R}^{N\times 1}$. 
            Then, an orthonormal basis for space $\mathcal{S}_H(N)$ can be given by the following lemma. 
            \begin{lemma}
                Matrices $\{\boldsymbol{B}_{1}, \ldots, \boldsymbol{B}_{N}; \boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}, 1\le n < l\le N\}$ form an orthonormal basis for $\mathcal{S}_H(N)$, which are defined as  
                \begin{subequations}\label{complm-def:herm-space-basis}
                    \begin{align}
                        \boldsymbol{B}_{n} & = \textup{diag}(\boldsymbol{b}_n), ~1\le n\le N, \label{complm-def:herm-space-diag-basis} \\
                        \boldsymbol{E}_{nl}^{(R)} & = \frac{1}{\sqrt{2}}\left(
                            \boldsymbol{e}_n\boldsymbol{e}_l^T + \boldsymbol{e}_l\boldsymbol{e}_n^T
                        \right), ~1\le n < l \le N, \label{complm-def:herm-space-real-basis} \\
                        \boldsymbol{E}_{nl}^{(I)} & = \frac{j}{\sqrt{2}}\left(
                            \boldsymbol{e}_n\boldsymbol{e}_l^T - \boldsymbol{e}_l\boldsymbol{e}_n^T
                        \right), ~1\le n < l \le N, \label{complm-def:herm-space-imag-basis}
                    \end{align}
                \end{subequations}
                where $\boldsymbol{e}_n\in\mathbb{R}^{N\times 1}$ has a $1$ for the $n$-th element and all other elements equal to zero. 
                More explicitly, $\boldsymbol{E}_{nl}^{(R)}$ and $\boldsymbol{E}_{nl}^{(I)}$ are defined as 
                \begin{subequations}\label{complm-def:nondiag-basis-explicit}
                    \allowdisplaybreaks
                    \begin{align}
                        \boldsymbol{E}_{nl}^{(R)} & = 
                            \frac{1}{\sqrt{2}}
                            \begin{blockarray}{*{5}{c} l}
                                \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
                                    $\ldots$ & $n$ & $\ldots$ & $l$ & $\ldots$ & \\
                                    \end{block}
                                    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                    \boldsymbol{0} & 0 & \boldsymbol{0} & 1 & \boldsymbol{0} & $n$ \\
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                    \boldsymbol{0} & 1 & \boldsymbol{0} & 0 & \boldsymbol{0} & $l$ \\
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                \end{block}
                            \end{blockarray},  \\
                        \boldsymbol{E}_{nl}^{(I)} & = 
                            \frac{1}{\sqrt{2}}
                            \begin{blockarray}{*{5}{c} l}
                                \begin{block}{*{5}{>{$\footnotesize}c<{$}} l}
                                    $\ldots$ & $n$ & $\ldots$ & $l$ & $\ldots$ & \\
                                    \end{block}
                                    \begin{block}{[*{5}{c}]>{$\footnotesize}l<{$}}
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                    \boldsymbol{0} & 0 & \boldsymbol{0} & j & \boldsymbol{0} & $n$ \\
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                    \boldsymbol{0} & -j & \boldsymbol{0} & 0 & \boldsymbol{0} & $l$ \\
                                    \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \boldsymbol{0} & \  \\
                                \end{block}
                            \end{blockarray}. 
                    \end{align}
                \end{subequations}
            \end{lemma}
            \begin{proof}[Proof\textup{:}\nopunct]
                It is easy to verify that these matrices are hermitian and orthonormal to each other under the Frobenius product $\text{tr}(\boldsymbol{A}^H\boldsymbol{B})$ for arbitrary $N\times N$ matrices $\boldsymbol{A}$ and $\boldsymbol{B}$. 
                Meanwhile, on one hand, for any $N\times N$ hermitian matrix $\boldsymbol{A}$, its main diagonal entries form an $N$-dimensional real vector, denoted as $\boldsymbol{d}_{\boldsymbol{A}} = \text{diag}(\boldsymbol{A})$. 
                Thus, there exists a real vector $\boldsymbol{c}_{\boldsymbol{A}} = [c_{\boldsymbol{A}, 1}, \ldots, c_{\boldsymbol{A}, N}]^T\in\mathbb{R}^{N\times 1}$ such that $\boldsymbol{d}_{\boldsymbol{A}} = \sum_{n = 1}^{N}{c_{\boldsymbol{A}, n}\boldsymbol{b}_n}$, i.e., 
                \begin{equation}\label{complm-eq:diag-vec-basis}
                    \text{diag}(\boldsymbol{d}_{\boldsymbol{A}}) = \sum_{n = 1}^{N}{c_{\boldsymbol{A}, n}\boldsymbol{B}_n}. 
                \end{equation}
                On the other hand, entries of matrices $\boldsymbol{E}_{nl}^{(R)}$ and $\boldsymbol{E}_{nl}^{(I)}$ are zero except for those on the $n$-th row, $l$-th column and $l$-th row, $n$-th column, $\forall n\neq l$. 
                Thus, it can be verified that $\boldsymbol{A}$ can be written as 
                \begin{equation}\label{complm-eq:herm-mat-basis-expansion}
                    \begin{aligned}
                        \boldsymbol{A} & = \sqrt{2}\sum_{n = 1}^{N - 1}\sum_{l = n + 1}^{N}{\text{Re}(A_{nl})\boldsymbol{E}_{nl}^{(R)} + \text{Im}(A_{nl})\boldsymbol{E}_{nl}^{(I)}} \\
                        & ~~~~ + \sum_{n = 1}^{N}{c_{\boldsymbol{A}, n}\boldsymbol{B}_{n}}, 
                    \end{aligned}
                \end{equation}
                which is the linear combination of $N(N - 1) + N = N^2$ matrices with $N^2$ real coefficients. 
                Therefore, the $N^2$ matrices $\{\boldsymbol{B}_1, \ldots, \boldsymbol{B}_{N}; \boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}$, $1\le n < l \le N\}$ form an orthonormal basis for the space of hermitian matrices. 
                % By relabeling these matrices as $\{\boldsymbol{O}_n$, $n = 1, \ldots, N^2\}$ and the corresponding coefficients as $r_1, \ldots, r_{N^2}$, matrix $\boldsymbol{A}$ can be written as equation~\eqref{eq:hermitian-coordinate}, and thus the lemma is proved. 
            \end{proof}
        
        
        \subsection{Dimension of Space $\mathcal{S}_X^{b}(N)$}\label{complm-subsec:spanned-space-dim}
            To show $\text{dim}(\mathcal{S}_X^{b}(N)) = \mathcal{D}_{N}^{(b)}$, we provide a two-fold proof, where we first prove $\text{dim}(\mathcal{S}_X^{b}(N)) \le \mathcal{D}_{N}^{(b)}$ and then $\text{dim}(\mathcal{S}_X^{b}(N)) \ge \mathcal{D}_{N}^{(b)}$. 

            For the first part, we show $\text{dim}(\mathcal{S}_X^{b}(N)) \le \mathcal{D}_{N}^{(b)}$. 
            Since $\mathcal{S}_X^{b}(N)$ is spanned by $\mathcal{S}_V^{b}(N)$ with real coefficients, we have $\mathcal{S}_X^{b}(N)\in\mathcal{S}_H(N)$ and thus $\text{dim}(\mathcal{S}_X^{b}(N))\le N^2$. 
            Due to the unit-amplitude of the IRS reflecting coefficients, however, the diagonal entries in any matrix $\boldsymbol{V}\in\mathcal{S}_V^{b}(N)$ are always equal to 1, i.e., $\text{diag}(\boldsymbol{V}) = \boldsymbol{1}_N = \sqrt{N}\boldsymbol{b}_1$. 
            Then, it is easy to verify that $\boldsymbol{V}$ is orthogonal to $\boldsymbol{B}_{2}, \ldots, \boldsymbol{B}_{N}$ for any values of $b$, i.e., 
            \begin{equation}\label{complm-eq:cov-null-space}
                \text{tr}(\boldsymbol{V}^H\boldsymbol{B}_{n}) = \sqrt{N}\boldsymbol{b}_{1}^T\boldsymbol{b}_{n} = 0, ~2\le n\le N. 
            \end{equation}
            Moreover, for $b = 1$, $\boldsymbol{V}$ is always a real matrix and thus we have $\text{tr}(\boldsymbol{V}^H\boldsymbol{E}_{nl}^{(I)}) = \text{Im}(V_{nl}) = 0$, $\forall n\neq l$. 
            Thus, for $b\ge 2$, $\mathcal{S}_X^{b}(N)$ should be a subspace of the space spanned by $\{\boldsymbol{B}_1; \boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}, 1\le n < l \le N\}$, leading to $\text{dim}(\mathcal{S}_X^{b}(N))\le N^2 - N + 1 = \mathcal{D}_{N}^{(b)}$, while for $b = 1$, $\mathcal{S}_X^{1}(N)$ should be a subspace of the space spanned by $\{\boldsymbol{B}_1; \boldsymbol{E}_{nl}^{(R)}, 1\le n < l \le N\}$, leading to $\text{dim}(\mathcal{S}_X^{1}(N))\le N(N - 1)/2 + 1 = \mathcal{D}_{N}^{(1)}$. 
            Therfore, $\text{dim}(\mathcal{S}_X^{b}(N))\le\mathcal{D}_{N}^{(b)}$ is proved for any positive integer $b$. 

            



            For the second part of the proof, we prove by induction. 
            To prove $\text{dim}(\mathcal{S}_X^{b}(N)) \ge \mathcal{D}_{N}^{(b)}$, it suffices to show that there exists at least $\mathcal{D}_{N}^{(b)}$ matrices in $\mathcal{S}_V^{b}(N)$ such that they are linearly independent with real coefficients. 
            For the following, we first prove the case with $b = 1$, and then consider the case with $b\ge 2$. 

            For $b = 1$, we show that there always exists $\mathcal{D}_{N}^{(1)} = (N^2 - N) / 2 + 1$ matrices in $\mathcal{S}_V^{1}(N)$ that are linearly independent with real coefficients. 
            It is easy to verify that this is true when $N \le 3$. 
            Assume that this is true for $N = L\ge 3$, and let $K_1 = \mathcal{D}_{L}^{(1)}$ for simplicity, then we have to show that this is true for $N = L + 1$. 
            Suppose $\boldsymbol{V}_k = \boldsymbol{v}_k\boldsymbol{v}_k^H$, $k = 1, \ldots, {K_1}$ are linearly independent matrices in $\mathcal{S}_V^{1}(L)$, where $\boldsymbol{v}_k\in{\{\pm 1\}}^L$, $k = 1, \ldots, K_1$. 
            Define matrix $\boldsymbol{W} = [\boldsymbol{v}_1, \ldots, \boldsymbol{v}_{K_1}]\in\mathbb{R}^{L\times {K_1}}$, which has full row rank $L$ according to the following lemma. 
            \begin{lemma}\label{complm-lemma:covariance-basis-full-rank}
                The matrix $\boldsymbol{W}$ has full row rank $L$ for $L\ge 3$. 
            \end{lemma}
            \begin{proof}[Proof of Lemma~\ref{complm-lemma:covariance-basis-full-rank}]
                Since $K_1 = \mathcal{D}_{L}^{(1)} > L$ for $L\ge 3$, we have $\text{rank}(\boldsymbol{W})\le L < {K_1}$. 
                If $\text{rank}(\boldsymbol{W}) < L$, then the space spanned by the columns of $\boldsymbol{W}$, denoted as $\text{span}(\boldsymbol{W})$, has a dimension lower than $L$. 
                Obviously, all vectors in $\{\pm 1\}^L$ spans the $L$-dimensional space $\mathbb{R}^L$, so there exists a vector $\boldsymbol{x}\in\{\pm 1\}^{L}$ such that $\boldsymbol{x}\notin\text{span}(\boldsymbol{W})$. 
                Let $\boldsymbol{x} = \boldsymbol{v}_{x} + \boldsymbol{y}$, where $\boldsymbol{v}_{x}\in\text{span}(\boldsymbol{W})$ while $\boldsymbol{y}\perp\text{span}(\boldsymbol{W})$. 
                Note that $\boldsymbol{X} = \boldsymbol{x}\boldsymbol{x}^H\in \mathcal{S}_V^{1}(N)$ and thus matrices $\{\boldsymbol{V}_1, \ldots, \boldsymbol{V}_{K_1}, \boldsymbol{X}\}$ must be linearly dependent with real coefficients according to the first part of the proof, because there are ${K_1} + 1 > \mathcal{D}_{L}^{(1)}$ symmetric matrices from $\mathcal{S}_V^{1}(N)$ in total. 
                Hence, there exists $\boldsymbol{\mu}\in\mathbb{R}^{{K_1}\times 1}$ and $\mu_x\in\mathbb{R}$, such that they are not all zeros and 
                \begin{equation}\label{complm-eq:mux-linear-dependent}
                    \mu_x\boldsymbol{X} + \sum_{k = 1}^{{K_1}}{\mu_k\boldsymbol{V}_k} = \boldsymbol{0}_{L\times L}. 
                \end{equation}
                Consider the matrix $\boldsymbol{Y} = \boldsymbol{y}\boldsymbol{y}^H$ and we have 
                \begin{subequations}\label{complm-eq:trace-applied}
                    \begin{align}
                        0 & = \text{tr}\left(
                            \boldsymbol{Y}^H\left(\mu_x\boldsymbol{X} + \sum_{k = 1}^{{K_1}}{\mu_k\boldsymbol{V}_k}\right)
                        \right) \\
                        & = \mu_x\text{tr}(\boldsymbol{Y}^H\boldsymbol{X}) + \sum_{k = 1}^{{K_1}}{\mu_k\text{tr}(\boldsymbol{Y}^H\boldsymbol{V}_k)}. 
                    \end{align}
                \end{subequations}
                Note that $\text{tr}(\boldsymbol{Y}^H\boldsymbol{X}) = |\boldsymbol{y}^H(\boldsymbol{v}_x + \boldsymbol{y})|^2 = \|\boldsymbol{y}\|_2^4$ and $\text{tr}(\boldsymbol{Y}^H\boldsymbol{V}_k) = |\boldsymbol{y}^H\boldsymbol{v}_k|^2 = 0$, $\forall k$. 
                Thus, equation~\eqref{complm-eq:trace-applied} is equivalent to $\mu_x\|\boldsymbol{y}\|_2^4 = 0$, which leads to $\mu_x = 0$ as $\boldsymbol{y}$ is nonzero. 
                Then, equation~\eqref{complm-eq:mux-linear-dependent} becomes $\sum_{k = 1}^{{K_1}}{\mu_k\boldsymbol{V}_k} = \boldsymbol{0}$ for some $\boldsymbol{\mu}\neq\boldsymbol{0}$. 
                This is contradictory to the assumption that $\{\boldsymbol{V}_k, k = 1, \ldots, {K_1}\}$ are linearly independent with real coefficients. 
                Therefore, $\boldsymbol{W}$ should have full row rank $L$. 
            \end{proof}
            Given Lemma~\ref{complm-lemma:covariance-basis-full-rank}, we implicitly construct $\mathcal{D}_{L + 1}^{(1)}$ linearly independent matrices in $S_V^1(L + 1)$ for the case of $N = L + 1$. 
            Define $(L + 1)$-dimensional vectors 
            \begin{equation}\label{complm-def:induction-construction}
                \boldsymbol{u}_{k} = [\boldsymbol{v}_k^T, 1]^T, \ \boldsymbol{y}_{k} = [-\boldsymbol{v}_k^T, 1]^T, \ k = 1, \ldots, {K_1}, 
            \end{equation}
            and matrices $\boldsymbol{U}_k = \boldsymbol{u}_k\boldsymbol{u}_k^H$ and $\boldsymbol{Y}_k = \boldsymbol{y}_k\boldsymbol{y}_k^H$, $\forall k$. 
            Obviously, $\boldsymbol{U}_k, \boldsymbol{Y}_k\in S_V^1(L + 1)$, $\forall k$, and there are $2{K_1} = 2\mathcal{D}_{L}^{(1)}$ matrices in total. 
            Note that for $L \ge 3$, we have $2\mathcal{D}_{L}^{(1)} > \mathcal{D}_{L + 1}^{(1)}$, so matrices $\{\boldsymbol{U}_k, \boldsymbol{Y}_k, k = 1, \ldots, {K_1}\}$ are linearly dependent with real coefficients according to the first part of the proof, i.e., there exists real vectors $\boldsymbol{\alpha} = [\alpha_1, \ldots, \alpha_{K_1}]^T, \boldsymbol{\beta} = [\beta_1, \ldots, \beta_{K_1}]^T\in\mathbb{R}^{{K_1}\times 1}$ such that 
            \begin{subequations}\label{complm-eq:induction-linearly-dependent-binary}
                \begin{align}
                    \boldsymbol{0} & = \sum_{k = 1}^{{K_1}}{\alpha_k\boldsymbol{U}_k + \beta_k\boldsymbol{Y}_k} \\
                    & = \sum_{k = 1}^{{K_1}}{
                        \left[
                            \begin{array}{cc}
                                (\alpha_k + \beta_k)\boldsymbol{v}_k\boldsymbol{v}_k^H & (\alpha_k - \beta_k)\boldsymbol{v}_k \\
                                (\alpha_k - \beta_k)\boldsymbol{v}_k^H & \alpha_k + \beta_k
                            \end{array}
                        \right]
                    }. 
                \end{align}
            \end{subequations}
            Thus, we have $\sum_{k = 1}^{{K_1}}{(\alpha_k + \beta_k)\boldsymbol{V}_k} = \boldsymbol{0}$. 
            However, $\{\boldsymbol{V}_k, k = 1, \ldots, {K_1}\}$ are linearly independent with real coefficients by assumption, which leads to $\boldsymbol{\alpha} + \boldsymbol{\beta} = \boldsymbol{0}$. 
            Therefore, $\sum_{k = 1}^{{K_1}}(\alpha_k - \beta_k)\boldsymbol{v}_k = 2\sum_{k = 1}^{{K_1}}{\alpha_k\boldsymbol{v}_k} = 2\boldsymbol{W}\boldsymbol{\alpha} = \boldsymbol{0}$. 
            Reversely, it is easy to verify that~\eqref{complm-eq:induction-linearly-dependent-binary} holds if $\boldsymbol{\alpha} + \boldsymbol{\beta} = \boldsymbol{0}$ and $\boldsymbol{W}\boldsymbol{\alpha} = \boldsymbol{0}$. 
            Thus,~\eqref{complm-eq:induction-linearly-dependent-binary} holds if and only if 
            \begin{equation}\label{complm-def:binary-null-space}
                \begin{aligned}
                    \left[
                        \begin{array}{c}
                            \boldsymbol{\alpha} \\
                            \boldsymbol{\beta}
                        \end{array}
                    \right] \in \mathcal{F} & = \bigg\{
                        \boldsymbol{x}\in\mathbb{R}^{2{K_1}\times 1} \bigg| \boldsymbol{x} = \left[
                            \begin{array}{c}
                                \boldsymbol{I}_{K_1\times K_1} \\
                                -\boldsymbol{I}_{K_1\times K_1}
                            \end{array}
                        \right]\boldsymbol{y}, \\
                        & ~~~~~~~~~~~~~~~~ \boldsymbol{y}\in\mathbb{R}^{{K_1}\times 1}, \ \boldsymbol{W}\boldsymbol{y} = \boldsymbol{0}
                    \bigg\}, 
                \end{aligned}
            \end{equation}
            where $\mathcal{F}$ is a subspace of $\mathbb{R}^{2{K_1}\times 1}$ and its dimension equals to that of the null space of $\boldsymbol{W}$, denoted as $\mathcal{N}(\boldsymbol{W})$, i.e., $\text{dim}(\mathcal{F}) = \text{dim}(\mathcal{N}(\boldsymbol{W})) = {K_1} - \text{rank}(\boldsymbol{W}) = {K_1} - L$. 
            Therefore, the maximum number of linearly independent matrices with real coefficients among $\{\boldsymbol{U}_k, \boldsymbol{Y}_k, k = 1, \ldots, {K_1}\}$, denoted as $M_1$, can be obtained as 
            \begin{equation}\label{eq:dim-construct-binary}
                    M_1 = 2{K_1} - \text{dim}(\mathcal{F}) = {K_1} + L. 
            \end{equation}
            As ${K_1} = \mathcal{D}_{L}^{(1)}$, we have $M_1 = (L^2 - L) / 2 + 1 + L = (L^2 + L) / 2 + 1 = \mathcal{D}_{L + 1}^{(1)}$. 
            Thus, there exists $\mathcal{D}_{L + 1}^{(1)}$ linearly independent matrices with real coefficients in the set $S_V^1(L + 1)$, which completes the proof of $\text{dim}(\mathcal{S}_{X}^{b}(N)) \ge \mathcal{D}_{N}^{(1)}$. 






            For $b \ge 2$, we have $\Phi_2 = \{\pm 1, \pm j\}\subseteq\Phi_b$ and $\mathcal{D}_{N}^{(b)} = \mathcal{D}_{N}^{(2)} = N^2 - N + 1$. 
            Therefore, it suffices to check the case of $b = 2$ only, i.e., showing that there always exists $\mathcal{D}_{N}^{(2)}$ matrices in $S_V^2(N)$ that are linearly independent with real coefficients. 
            Then, for any $b\ge 2$, the same matrices can be found in $\mathcal{S}_V^{b}(N)$ such that they are linearly independent with real coefficients. 

            For $b = 2$, it is easy to verify the cases where $N \le 3$. 
            Assume that for $N = L\ge 3$, there exists $K_2 = \mathcal{D}_{L}^{(2)} = L^2 - L + 1$ matrices in $S_V^2(L)$ that are linearly independent with real coefficients, which are denoted as $\boldsymbol{V}_k = \boldsymbol{v}_k\boldsymbol{v}_k^H$, $k = 1, \ldots, K_2$, with $\boldsymbol{v}_k\in{\{\pm 1, \pm j\}}^L$, $\forall k$. 
            Similar to the case of $b = 1$, we implicitly construct $\mathcal{D}_{L + 1}^{(2)}$ linearly independent matrices in $S_V^2(L + 1)$ to prove the case of $N = L + 1$. 
            Specifically, define $\boldsymbol{d}_k = (1 - j)\boldsymbol{v}_k\in\{1+j, 1-j, -1+j, -1-j\}^L$, $k = 1, \ldots, K$, then we have $\boldsymbol{V}_k = \boldsymbol{d}_k\boldsymbol{d}_k^H / 2, \forall k$. 
            Note that the real and imaginary parts of vector $\boldsymbol{d}_k$ can be considered as two binary variables independent of each other. 
            Thus, it can be decomposed into two parts, i.e., $\boldsymbol{d}_k = \boldsymbol{d}_{k, r} + j\boldsymbol{d}_{k, i}$, where $\boldsymbol{d}_{k, r}, \boldsymbol{d}_{k, i}\in\{\pm 1\}^L = \Phi_1^L$. 
            Consider vectors $\boldsymbol{q}_k = [\boldsymbol{d}_{k, r}^T, \boldsymbol{d}_{k, i}^T]^T\in\{\pm 1\}^{2L}$, $k = 1, \ldots, {K_2}$. 
            Let matrix $\boldsymbol{Q} = [\boldsymbol{q}_1, \ldots, \boldsymbol{q}_{K_2}]\in\mathbb{R}^{2L\times {K_2}}$, and $R = 2L - \text{rank}(\boldsymbol{Q}) \ge 0$. 
            If $R > 0$, i.e., $\text{rank}(\boldsymbol{Q}) < 2L$, there exists vectors $\boldsymbol{q}_{{K_2} + 1}, \ldots, \boldsymbol{q}_{{K_2} + R}\in\{\pm 1\}^{2L}$ such that $\tilde{\boldsymbol{Q}} = [\boldsymbol{Q}, \boldsymbol{q}_{{K_2} + 1}, \ldots, \boldsymbol{q}_{{K_2} + R}]\in\mathbb{R}^{2L\times({K_2} + R)}$ has full row rank $2L$. 
            Correspondingly, for $k = {K_2} + 1, \ldots, {K_2} + R$, we decompose $\boldsymbol{q}_{k}$ as $\boldsymbol{q}_{k} = [\boldsymbol{d}_{k, r}^T, \boldsymbol{d}_{k, i}^T]^T$ with $\boldsymbol{d}_{k, r}, \boldsymbol{d}_{k, i}\in\mathbb{R}^{L\times 1}$ and define $\boldsymbol{d}_k = \boldsymbol{d}_{k, r} + j\boldsymbol{d}_{k, i}$ and $\boldsymbol{v}_k = \boldsymbol{d}_k / (1 - j)\in\Phi_2^{L}$. 
            If $R = 0$, however, let $\tilde{\boldsymbol{Q}} = \boldsymbol{Q}$. 
            
            For $N = L + 1$, consider $(L + 1)$-dimensional vectors 
            \begin{equation}
                \boldsymbol{u}_k = [\boldsymbol{v}_k^T, 1]^T, \ \boldsymbol{y}_k = [-\boldsymbol{v}_k^T, 1]^T, \ k = 1, \ldots, {K_2} + R, 
            \end{equation}
            and matrices $\boldsymbol{U}_k = \boldsymbol{u}_k\boldsymbol{u}_k^H$ and $\boldsymbol{Y}_k = \boldsymbol{y}_k\boldsymbol{y}_k^H$, which are included in $S_V^2(L + 1)$, and there are $2({K_2} + R)$ matrices in total. 
            As we have $2({K_2} + R) \ge 2{K_2} > \mathcal{D}_2(L + 1)$, they must be linearly dependent over $\mathbb{R}$ according to the first part of the proof. 
            There exists real vectors $\boldsymbol{\alpha} = [\alpha_1, \ldots, \alpha_{{K_2} + R}]^T, \boldsymbol{\beta} = [\beta_1, \ldots, \beta_{{K_2} + R}]^T\in\mathbb{R}^{({K_2} + R)\times 1}$ such that 
            \begin{subequations}\label{eq:induction-linearly-dependent-multiary}
                \begin{align}
                    \boldsymbol{0} & = \sum_{k = 1}^{{K_2} + R}{\alpha_k\boldsymbol{U}_k + \beta_k\boldsymbol{Y}_k} \\
                    & = \sum_{k = 1}^{{K_2} + R}{\left[
                        \begin{array}{cc}
                            (\alpha_k + \beta_k)\boldsymbol{v}_k\boldsymbol{v}_k^H & (\alpha_k - \beta_k)\boldsymbol{v}_k \\
                            (\alpha_k - \beta_k)\boldsymbol{v}_k^H & \alpha_k + \beta_k
                        \end{array}
                    \right]}. 
                \end{align}
            \end{subequations}
            Define $\mathcal{G}_{s}$ as the set of all vectors $\boldsymbol{s}\in\mathbb{R}^{(K_2 + R)\times 1}$ such that $\sum_{k = 1}^{{K_2} + R}{s_k\boldsymbol{V}_k} = \boldsymbol{0}$ holds, then $\boldsymbol{\alpha} + \boldsymbol{\beta}\in\mathcal{G}_{s}$. 
            Since $\boldsymbol{V}_1, \ldots, \boldsymbol{V}_{K_2}$ are linearly independent, $\mathcal{G}_s$ is a linear space of which the dimension is bounded by $\text{dim}(\mathcal{G}_s)\le {K_2} + R - {K_2} = R$. 
            On the other hand, let $\boldsymbol{z} = \boldsymbol{\alpha} - \boldsymbol{\beta}$ and we have $\sum_{k = 1}^{{K_2} + R}{z_k\boldsymbol{v}_k} = \boldsymbol{0}$, so $\sum_{k = 1}^{{K_2} + R}{z_k\boldsymbol{d}_k} = (1 - j)\sum_{{K_2} = 1}^{K + R}{z_k\boldsymbol{v}_k} = \boldsymbol{0}$. 
            As $\boldsymbol{z}$ is a real vector, we have 
            \begin{equation}
                \tilde{\boldsymbol{Q}}\boldsymbol{z} = \sum_{k = 1}^{{K_2} + R}{z_k\left[
                    \begin{array}{c}
                        \boldsymbol{d}_{k, r} \\
                        \boldsymbol{d}_{k, i}
                    \end{array}
                \right]} = \sum_{k = 1}^{{K_2} + R}\left[
                    \begin{array}{c}
                        {z_k\text{Re}(\boldsymbol{d}_{k})} \\
                        {z_k\text{Im}(\boldsymbol{d}_{k})}
                    \end{array}
                \right] = \boldsymbol{0}, 
            \end{equation}
            which means $\boldsymbol{z}$ is in the null space of $\tilde{\boldsymbol{Q}}$, i.e., $\mathcal{N}(\tilde{\boldsymbol{Q}})$. 
            The dimension of $\mathcal{N}(\tilde{\boldsymbol{Q}})$ is ${K_2} + R - 2L$, because $\tilde{\boldsymbol{Q}}\in\mathbb{R}^{2L\times ({K_2} + R)}$ has full row rank $2L$ by definition. 
            Reversely, one can easily verify that equation~\eqref{eq:induction-linearly-dependent-multiary} is true as long as $\boldsymbol{\alpha} + \boldsymbol{\beta}\in{\mathcal{G}_s}$ and $\boldsymbol{\alpha} - \boldsymbol{\beta}\in\mathcal{N}(\tilde{\boldsymbol{Q}})$. 
            Therefore, $\sum_{k = 1}^{{K_2} + R}{\alpha_k\boldsymbol{U}_k + \beta_k\boldsymbol{Y}_k} = \boldsymbol{0}$ if and only if $\boldsymbol{\alpha} + \boldsymbol{\beta}\in\mathcal{G}_s$ and $\boldsymbol{\alpha} - \boldsymbol{\beta}\in\mathcal{N}(\tilde{\boldsymbol{Q}})$, i.e., 
            \begin{equation}
                \begin{aligned}
                    \left[
                        \begin{array}{c}
                            \boldsymbol{\alpha} + \boldsymbol{\beta} \\
                            \boldsymbol{\alpha} - \boldsymbol{\beta}
                        \end{array}
                    \right] \in\mathcal{G} & = \bigg\{
                        \boldsymbol{x}\in\mathbb{R}^{2({K_2} + R)\times 1}\bigg|
                            \boldsymbol{x} = \left[
                                \begin{array}{c}
                                    \boldsymbol{s} \\
                                    \boldsymbol{z}
                                \end{array}
                            \right], \\
                            & ~~~~~~~~~~~~~~~~~ \boldsymbol{s}\in\mathcal{G}_s, \ \boldsymbol{z}\in\mathcal{N}(\tilde{\boldsymbol{Q}})
                    \bigg\}, 
                \end{aligned}
            \end{equation}
            where $\mathcal{G}$ is a subspace of $\mathbb{R}^{2({K_2} + R)\times 1}$. 
            Note that 
            \begin{equation}
                \left[
                    \begin{array}{c}
                        \boldsymbol{\alpha} \\
                        \boldsymbol{\beta}
                    \end{array}
                \right] = \frac{1}{2}\left[
                    \begin{array}{cc}
                        \boldsymbol{I} & \boldsymbol{I} \\
                        \boldsymbol{I} & -\boldsymbol{I}
                    \end{array}
                \right]\left[
                    \begin{array}{c}
                        \boldsymbol{\alpha} + \boldsymbol{\beta} \\
                        \boldsymbol{\alpha} - \boldsymbol{\beta}
                    \end{array}
                \right], 
            \end{equation}
            where the transformation matrix is invertible, so the dimension of the solution space of $[\boldsymbol{\alpha}^T, \boldsymbol{\beta}^T]^T$ for~\eqref{eq:induction-linearly-dependent-multiary} equals to the dimension of $\mathcal{G}$. 
            Thus, the maximum number $M_2$ of linearly independent matrices among $\{\boldsymbol{U}_k, \boldsymbol{Y}_k, k = 1, \ldots, {K_2} + R\}$ over $\mathbb{R}$ can be obtained as
            \begin{subequations}\label{eq:dim-construct-multiary}
                \begin{align}
                    M_2 & = 2({K_2} + R) - \text{dim}(\mathcal{G}) \\
                    & = 2({K_2} + R) - (\text{dim}(\mathcal{G}_s) + \text{dim}(\mathcal{N}(\tilde{\boldsymbol{Q}}))) \\
                    & \ge 2({K_2} + R) - (R + {K_2} + R - 2L) \\
                    & = {K_2} + 2L. 
                \end{align}
            \end{subequations}
            As ${K_2} = \mathcal{D}_{L}^{(2)} = L^2 - L + 1$, we have $M_2 \ge {K_2} + 2L = L^2 + L + 1 = \mathcal{D}_2(L + 1)$. 
            Therefore, there exists at least $\mathcal{D}_2(L + 1)$ linearly independent matrices in the set $S_V^2(L + 1)$, which completes the proof of $T_X^b(N)\ge\mathcal{D}_{N}^{(b)}$ for the $b = 2$ case, and thus the $b\ge 2$ case. 

            Combining two parts of the proof, i.e., $T_X^b(N)\le\mathcal{D}_{N}^{(b)}$ and $T_X^b(N)\ge\mathcal{D}_{N}^{(b)}$, we conclude that $T_X^b(N) = \mathcal{D}_{N}^{(b)}$, which completes the proof of equation~\eqref{def:spanned-spaced-dimension}. 
            Additionally, for $b\ge 2$, it has been shown that $\mathcal{S}_X^{b}(N)$ is a subspace of the space spanned by $\{\boldsymbol{B}_1; \boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}, 1\le n < l \le N\}$ over $\mathbb{R}$, whose dimension is $N^2 - N + 1$, which is the same as the dimension of $\mathcal{S}_X^{b}(N)$, i.e., $T_X^b(N)$ proved above. 
            Hence, $\mathcal{S}_X^{b}(N)$ equals to the spanned space and $\{\boldsymbol{B}_1; \boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}, 1\le n < l \le N\}$ is one set of orthonormal basis of $\mathcal{S}_X^{b}(N)$ for $b\ge 2$. 
            Similarly, one set of orthonormal basis of $\mathcal{S}_X^{b}(N)$ for $b = 1$ is given by $\{\boldsymbol{B}_1; \boldsymbol{E}_{nl}^{(R)}, 1\le n < l \le N\}$. 

        Proposition~\ref{prop:spanned-space-dimension} explicitly specifies the dimension of the linear space spanned by the autocorrelation matrices of IRS reflection vectors subject to discrete phase shift constraint, as well as the orthonormal basis of the space. 
        In the following subsection, the uniqueness of the channel autocorrelation matrix for sufficiently large $N$ and $T_{p}$ is analyzed by utilizing the orthonormal basis given in the proposition. 

    \subsection{Uniqueness of Channel Autocorrelation Matrix}\label{subsec:csi-cov-uniqueness}
        Suppose $T_{p}\ge T_X^b(N)$ and any $T_X^b(N)$ matrices among $\{\boldsymbol{V}_t, t = 1, \ldots, T_{p}\}$ are linearly independent over $\mathbb{R}$. 
        Then, the power measurements $p_t = \text{tr}(\boldsymbol{H}\boldsymbol{V}_t), t = 1, \ldots, T_{p}$ can be seen as the projection of the matrix $\boldsymbol{H}$ into the space $\mathcal{S}_X^{b}(N)$. 

        For $b\ge 2$, it is easy to verify that $\bar{\boldsymbol{H}} = \bar{\boldsymbol{h}}\bar{\boldsymbol{h}}^H$ is a solution to Problem~\eqref{prob:cov-est-find-origin}. 
        Suppose there exists a matrix $\hat{\boldsymbol{H}}\neq\bar{\boldsymbol{H}}$ that is also a solution to Problem~\eqref{prob:cov-est-find-origin}. 
        Then, $\hat{\boldsymbol{H}}$ is a rank-one hermitian matrix and we have $\text{tr}(\hat{\boldsymbol{H}}\boldsymbol{V}_t) = p_t = \text{tr}(\bar{\boldsymbol{H}}\boldsymbol{V}_t)$, $t = 1, \ldots, T_{p}$. 
        Define $\hat{\boldsymbol{H}} = \hat{\boldsymbol{h}}\hat{\boldsymbol{h}}^H$ and $\mathcal{\boldsymbol{E}} = \bar{\boldsymbol{H}} - \hat{\boldsymbol{H}}\in\mathbb{C}^{N\times N}$, then we have $\text{rank}(\mathcal{\boldsymbol{E}})\le 2$ and $\text{tr}(\mathcal{\boldsymbol{E}}\boldsymbol{V}_t) = 0$ for $\forall t$. 
        With $T_{p}\ge T_X^b(N)$, the matrix $\mathcal{\boldsymbol{E}}$ is perpendicular to the space $\mathcal{S}_X^{b}(N)$, which results in $\text{tr}(\mathcal{\boldsymbol{E}}\boldsymbol{E}_{nl}^{(R)}) = \text{tr}(\mathcal{\boldsymbol{E}}\boldsymbol{E}_{nl}^{(I)}) = 0$, $1\le n < l\le N$, and also $\text{tr}(\mathcal{\boldsymbol{E}}\boldsymbol{B}_{1}) = \text{tr}(\mathcal{\boldsymbol{E}})/\sqrt{N} = 0$. 
        According to the definitions of matrices $\boldsymbol{E}_{nl}^{(R)}, \boldsymbol{E}_{nl}^{(I)}, 1\le n < l\le N$, we have 
        \begin{equation}\label{eq:sol-err-multiary}
            \begin{aligned}
                \mathcal{\boldsymbol{E}} & = 
                    \left[
                        \begin{array}{cccc}
                            \mathcal{E}_{11} & 0 & \ldots & 0 \\
                            0 & \mathcal{E}_{22} & \ldots & 0 \\
                            \vdots & \vdots & \ddots & 0 \\
                            0 & 0 & 0 & \mathcal{E}_{NN}
                        \end{array}
                    \right], 
            \end{aligned}
        \end{equation}
        where $\mathcal{E}_{nn} = |\bar{h}_n|^2 - |\hat{h}_n|^2$. 
        Because of $\text{rank}(\mathcal{\boldsymbol{E}})\le 2$, we have $\mathcal{E}_{nn} = 0$ for $n\ge 3$ without loss of generality, and thus $|\bar{h}_n| = |\hat{h}_n|$ for $n\ge 3$. 
        % By assuming $N\ge 3$, we have $\mathcal{E}_{31} = 0 = \bar{h}_3\bar{h}_1^* - \hat{h}_3\hat{h}_1^*$, leading to $|\bar{h}_3\bar{h}_1| = |\hat{h}_3\hat{h}_1|$. 
        % Since $\bar{h}_3\neq 0$ holds with probability $1$, we find that $|\bar{h}_1| = |\hat{h}_1|$. 
        % Similarly, $|\bar{h}_2| = |\hat{h}_2|$ can be obtained from $\mathcal{E}_{32} = 0$. 
        By assuming $N\ge 3$, we have $\mathcal{E}_{n1} = \bar{h}_n\bar{h}_1^* - \hat{h}_n\hat{h}_1^* = 0$, $n = 3, \ldots, N$, leading to $|\bar{h}_n\bar{h}_1| = |\hat{h}_n\hat{h}_1|$ for $\forall n\ge 3$. 
        Since $\bar{h}_n \neq 0$ holds with probability $1$ for $\forall n$, we find that $|\bar{h}_1| = |\hat{h}_1|$. 
        Similarly, $|\bar{h}_2| = |\hat{h}_2|$ can be obtained. 
        Then, $\mathcal{E}_{11} = \mathcal{E}_{22} = 0$ and thus $\mathcal{\boldsymbol{E}} = \boldsymbol{0}$, which indicates $\bar{\boldsymbol{H}} = \hat{\boldsymbol{H}}$. 
        Hence, $\bar{\boldsymbol{H}}$ is the unique solution to Problem~\eqref{prob:cov-est-find-origin} with probability $1$ when $b\ge 2$, $N\ge 3$ and $T_{p}$ is sufficiently large. 

        For $b = 1$, the IRS reflection vectors are all real vectors and we have $p_t = \text{tr}(\boldsymbol{H}\boldsymbol{V}_t) = \text{tr}(\text{Re}(\boldsymbol{H})\boldsymbol{V}_t)$, $t = 1, \ldots, T_{p}$. 
        It is easy to verify that both $\bar{\boldsymbol{H}}$ and $\bar{\boldsymbol{H}}^*$ are the solutions to Problem~\eqref{prob:cov-est-find-origin}. 
        Recall that $\bar{\boldsymbol{H}}_r = \text{Re}(\bar{\boldsymbol{H}}) = \text{Re}(\bar{\boldsymbol{H}}^*)$ is the real part of the solutions. 
        Suppose there exists a matrix $\hat{\boldsymbol{H}}$ that does not equal to $\bar{\boldsymbol{H}}$ or $\bar{\boldsymbol{H}}^*$ but is also a solution to Problem~\eqref{prob:cov-est-find-origin}, and its real part is denoted as $\hat{\boldsymbol{H}}_r = \text{Re}(\hat{\boldsymbol{H}})$. 
        Obviously, the ranks of both $\bar{\boldsymbol{H}}_r$ and $\hat{\boldsymbol{H}}_r$ are no more than two. 
        Similar to the case where $b\ge 2$, we define $\mathcal{\boldsymbol{E}}_r = \bar{\boldsymbol{H}}_r - \hat{\boldsymbol{H}}_r\in\mathbb{R}^{N\times N}$, which is a real symmetric matrix satisfying $\text{rank}(\mathcal{\boldsymbol{E}}_r)\le 4$. 
        Thus, we have $\text{tr}(\mathcal{\boldsymbol{E}}_r\boldsymbol{V}_t) = 0$, $t = 1, \ldots, T_{p}$. 
        Since $T_{p}\ge T_X^b(N)$, the matrix $\mathcal{\boldsymbol{E}}$ is perpendicular to the space $\mathcal{S}_X^{b}(N)$ and thus $\text{tr}(\mathcal{\boldsymbol{E}}\boldsymbol{E}_{nl}^{(R)}) = 0$, $1\le n < l\le N$. 
        As a result, $\mathcal{\boldsymbol{E}}_r$ can be written as 
        \begin{equation}\label{eq:sol-err-binary}
            \begin{aligned}
                \mathcal{\boldsymbol{E}}_r & = 
                    \left[
                        \begin{array}{cccc}
                            \mathcal{E}_{r, 11} & 0 & \ldots & 0 \\
                            0 & \mathcal{E}_{r, 22} & \ldots & 0 \\
                            \vdots & \vdots & \ddots & 0 \\
                            0 & 0 & 0 & \mathcal{E}_{r, NN}
                        \end{array}
                    \right], 
            \end{aligned}
        \end{equation}
        where $\mathcal{E}_{r, nn}$ is the $n$-th diagonal element of $\mathcal{\boldsymbol{E}}_r$. 
        Without loss of generality, we have $\mathcal{E}_{r, nn} = 0$ for $n\ge 5$ due to $\text{rank}(\mathcal{\boldsymbol{E}}_r)\le 4$. 
        Since $\bar{\boldsymbol{H}} = \bar{\boldsymbol{h}}\bar{\boldsymbol{h}}^H$, it is easy to verify that $\bar{\boldsymbol{H}}_r = \bar{\boldsymbol{h}}_{r}\bar{\boldsymbol{h}}_{r}^T + \bar{\boldsymbol{h}}_{m}\bar{\boldsymbol{h}}_{m}^T$, where $\bar{\boldsymbol{h}}_{r} = \text{Re}(\bar{\boldsymbol{h}})$ and $\bar{\boldsymbol{h}}_{m} = \text{Im}(\bar{\boldsymbol{h}})$. 
        Similarly, by defining $\hat{\boldsymbol{H}} = \hat{\boldsymbol{h}}\hat{\boldsymbol{h}}^H$, we have $\hat{\boldsymbol{H}}_r = \hat{\boldsymbol{h}}_{r}\hat{\boldsymbol{h}}_{r}^T + \hat{\boldsymbol{h}}_{m}\hat{\boldsymbol{h}}_{m}^T$, where $\hat{\boldsymbol{h}}_{r} = \text{Re}(\hat{\boldsymbol{h}})$ and $\hat{\boldsymbol{h}}_{m} = \text{Im}(\hat{\boldsymbol{h}})$. 
        Consider real matrices
        \begin{subequations}\label{def:csi-seg-binary}
            \begin{align}
                \bar{\boldsymbol{A}} & = 
                    \left[
                        \begin{array}{cc}
                            \bar{h}_{r, 1} & \bar{h}_{m, 1} \\
                            \vdots    & \vdots    \\
                            \bar{h}_{r, 4} & \bar{h}_{m, 4}
                        \end{array}
                    \right], 
                & \hat{\boldsymbol{A}} & = 
                \left[
                    \begin{array}{cc}
                        \hat{h}_{r, 1} & \hat{h}_{m, 1} \\
                        \vdots    & \vdots    \\
                        \hat{h}_{r, 4} & \hat{h}_{m, 4}
                    \end{array}
                \right], \\
                \bar{\boldsymbol{B}} & = 
                    \left[
                        \begin{array}{cc}
                            \bar{h}_{r, 5} & \bar{h}_{m, 5} \\
                            \vdots    & \vdots    \\
                            \bar{h}_{r, N} & \bar{h}_{m, N}
                        \end{array}
                    \right], 
                & \hat{\boldsymbol{B}} & = 
                \left[
                    \begin{array}{cc}
                        \hat{h}_{r, 5} & \hat{h}_{m, 5} \\
                        \vdots    & \vdots    \\
                        \hat{h}_{r, N} & \hat{h}_{m, N}
                    \end{array}
                \right], 
            \end{align}
        \end{subequations}
        where $\bar{h}_{r, n}$, $\bar{h}_{m, n}$, $\hat{h}_{r, n}$ and $\hat{h}_{m, n}$ are the $n$-th elements of vectors $\bar{\boldsymbol{h}}_{r}$, $\bar{\boldsymbol{h}}_{m}$, $\hat{\boldsymbol{h}}_{r}$ and $\hat{\boldsymbol{h}}_{m}$, respectively. 
        Then, the matrix $\mathcal{\boldsymbol{E}}_r$ can be equivalently written as 
        \begin{subequations}\label{eq:err-mat-block-binary}
            \begin{align}
                \mathcal{\boldsymbol{E}}_r & = \bar{\boldsymbol{H}}_r - \hat{\boldsymbol{H}}_r \\
                & = 
                \left[
                    \begin{array}{c}
                        \bar{\boldsymbol{A}} \\
                        \bar{\boldsymbol{B}}
                    \end{array}
                \right]\left[
                    \bar{\boldsymbol{A}}^T, \bar{\boldsymbol{B}}^T
                \right] - \left[
                    \begin{array}{c}
                        \hat{\boldsymbol{A}} \\
                        \hat{\boldsymbol{B}}
                    \end{array}
                \right]\left[
                    \hat{\boldsymbol{A}}^T, \hat{\boldsymbol{B}}^T
                \right] \\
                & = \left[
                    \begin{array}{cc}
                        \bar{\boldsymbol{A}}\bar{\boldsymbol{A}}^T - \hat{\boldsymbol{A}}\hat{\boldsymbol{A}}^T & \bar{\boldsymbol{A}}\bar{\boldsymbol{B}}^T - \hat{\boldsymbol{A}}\hat{\boldsymbol{B}}^T \\
                        \bar{\boldsymbol{B}}\bar{\boldsymbol{A}}^T - \hat{\boldsymbol{B}}\hat{\boldsymbol{A}}^T & \bar{\boldsymbol{B}}\bar{\boldsymbol{B}}^T - \hat{\boldsymbol{B}}\hat{\boldsymbol{B}}^T
                    \end{array}
                \right], \label{eq:err-block-binary}
            \end{align}
        \end{subequations}
        where $\bar{\boldsymbol{A}}\bar{\boldsymbol{A}}^T - \hat{\boldsymbol{A}}\hat{\boldsymbol{A}}^T$ is a $4\times 4$ diagonal matrix and all other three blocks in~\eqref{eq:err-block-binary} are zeros, according to equation~\eqref{eq:sol-err-binary} and the analysis above. 
        Thus, we have $\bar{\boldsymbol{A}}\bar{\boldsymbol{B}}^T = \hat{\boldsymbol{A}}\hat{\boldsymbol{B}}^T$ and $\bar{\boldsymbol{B}}\bar{\boldsymbol{B}}^T = \hat{\boldsymbol{B}}\hat{\boldsymbol{B}}^T$. 
        Obviously, the space spanned by the columns of $\hat{\boldsymbol{B}}$ is the same as that of $\bar{\boldsymbol{B}}$, which means the columns of $\hat{\boldsymbol{B}}$ can be represented by $\bar{\boldsymbol{B}}$ with a coefficient matrix $\boldsymbol{Y}\in\mathbb{R}^{2\times 2}$, i.e., $\hat{\boldsymbol{B}} = \bar{\boldsymbol{B}}\boldsymbol{Y}$. 
        Thus, $\bar{\boldsymbol{B}}\bar{\boldsymbol{B}}^T = \hat{\boldsymbol{B}}\hat{\boldsymbol{B}}^T = \bar{\boldsymbol{B}}\boldsymbol{Y}\boldsymbol{Y}^T\bar{\boldsymbol{B}}^T$. 
        Since $\bar{\boldsymbol{h}}$ represents the equivalent channel from the BS to user, the matrix $\bar{\boldsymbol{B}}$ has full column rank $2$ with probability $1$ for $N\ge 6$, and thus $\bar{\boldsymbol{B}}^T\bar{\boldsymbol{B}}\in\mathbb{R}^{2\times 2}$ is invertible. 
        Hence, $\boldsymbol{Y}\boldsymbol{Y}^T$ can be solved as
        \begin{equation}
            \boldsymbol{Y}\boldsymbol{Y}^T = \left(\bar{\boldsymbol{B}}^T\bar{\boldsymbol{B}}\right)^{-1}\bar{\boldsymbol{B}}^T\left(\bar{\boldsymbol{B}}\bar{\boldsymbol{B}}^T\right)\bar{\boldsymbol{B}}\left(\bar{\boldsymbol{B}}^T\bar{\boldsymbol{B}}\right)^{-1} = \boldsymbol{I}, 
        \end{equation}
        which means that $\boldsymbol{Y}\in\mathbb{R}^{2\times 2}$ is an orthogonal matrix. 
        On the other hand, we have $\bar{\boldsymbol{A}}\bar{\boldsymbol{B}}^T = \hat{\boldsymbol{A}}\hat{\boldsymbol{B}}^T = \hat{\boldsymbol{A}}\boldsymbol{Y}^T\bar{\boldsymbol{B}}^T$. 
        By applying $\bar{\boldsymbol{B}}$ on the left to both sides, it can be simplified as $\bar{\boldsymbol{A}} = \hat{\boldsymbol{A}}\boldsymbol{Y}^T$, or equivalently, $\hat{\boldsymbol{A}} = \bar{\boldsymbol{A}}\boldsymbol{Y}$. 
        Then, $\bar{\boldsymbol{A}}\bar{\boldsymbol{A}}^T = \hat{\boldsymbol{A}}\boldsymbol{Y}^T\boldsymbol{Y}\hat{\boldsymbol{A}}^T = \hat{\boldsymbol{A}}\hat{\boldsymbol{A}}^T$ holds and $\mathcal{\boldsymbol{E}}_r = \boldsymbol{0}$ follows, which leads to $\bar{\boldsymbol{H}}_r = \hat{\boldsymbol{H}}_r$. 
        Moreover, it is worth noting that
        \begin{equation}
            \bar{\boldsymbol{h}} = \left[
                \bar{\boldsymbol{h}}_{r}, \bar{\boldsymbol{h}}_{m}
            \right]\left[
                \begin{array}{c}
                    1 \\
                    j
                \end{array}
            \right] = \left[
                \begin{array}{c}
                    \bar{\boldsymbol{A}} \\
                    \bar{\boldsymbol{B}}
                \end{array}
            \right]\left[
                \begin{array}{c}
                    1 \\
                    j
                \end{array}
            \right]. 
        \end{equation}
        Therefore, the matrix $\bar{\boldsymbol{H}}$ can be written as 
        \begin{equation}
            \bar{\boldsymbol{H}} = \bar{\boldsymbol{h}}\bar{\boldsymbol{h}}^H = \left[
                \begin{array}{c}
                    \bar{\boldsymbol{A}} \\
                    \bar{\boldsymbol{B}}
                \end{array}
            \right]\left[
                \begin{array}{cc}
                    1 & -j \\
                    j &  1
                \end{array}
            \right]\left[
                \bar{\boldsymbol{A}}^T, \bar{\boldsymbol{B}}^T
            \right]. 
        \end{equation}
        Similarly, $\hat{\boldsymbol{H}}$ can be equivalently written as
        \begin{subequations}
            \begin{align}
                \hat{\boldsymbol{H}} & = \left[
                    \begin{array}{c}
                        \hat{\boldsymbol{A}} \\
                        \hat{\boldsymbol{B}}
                    \end{array}
                \right]\left[
                    \begin{array}{cc}
                        1 & -j \\
                        j &  1
                    \end{array}
                \right]\left[
                        \hat{\boldsymbol{A}}^T, \hat{\boldsymbol{B}}^T
                \right] \\
                % & = \left[
                %     \begin{array}{c}
                %         \bar{\boldsymbol{A}}\boldsymbol{Y} \\
                %         \bar{\boldsymbol{B}}\boldsymbol{Y}
                %     \end{array}
                % \right]\left[
                %     \begin{array}{cc}
                %         1 & -j \\
                %         j &  1
                %     \end{array}
                % \right]\left[
                %     \boldsymbol{Y}^T\bar{\boldsymbol{A}}^T, \boldsymbol{Y}^T\bar{\boldsymbol{B}}^T
                % \right] \\
                & = \left[
                    \begin{array}{c}
                        \bar{\boldsymbol{A}} \\
                        \bar{\boldsymbol{B}}
                    \end{array}
                \right]\boldsymbol{Y}\left[
                    \begin{array}{cc}
                        1 & -j \\
                        j &  1
                    \end{array}
                \right]\boldsymbol{Y}^T\left[
                    \bar{\boldsymbol{A}}^T, \bar{\boldsymbol{B}}^T
                \right]. 
            \end{align}
        \end{subequations}
        Define matrix $\boldsymbol{J}\in\mathbb{R}^{2\times 2}$ as 
        \begin{equation}
            \boldsymbol{J} = \boldsymbol{Y}\left[
                    \begin{array}{cc}
                        1 & -j \\
                        j &  1
                    \end{array}
                \right]\boldsymbol{Y}^T. 
        \end{equation}
        Let $\boldsymbol{Y} = [\boldsymbol{y}_1, \boldsymbol{y}_2]$ with $\boldsymbol{y}_1 = [y_{11}, y_{12}]^T$ and $\boldsymbol{y}_2 = [y_{21}, y_{22}]^T$. 
        Then, we have $\boldsymbol{y}_1\boldsymbol{y}_1^T + \boldsymbol{y}_2\boldsymbol{y}_2^T = \boldsymbol{Y}\boldsymbol{Y}^T = \boldsymbol{I}$ and
        \begin{subequations}
            \begin{align}
                \boldsymbol{J} & = \left(\boldsymbol{y}_1 + j\boldsymbol{y}_2\right)\left(\boldsymbol{y}_1^T - j\boldsymbol{y}_2^T\right) \\
                & = \left(\boldsymbol{y}_1\boldsymbol{y}_1^T + \boldsymbol{y}_2\boldsymbol{y}_2^T\right) + j\left(\boldsymbol{y}_2\boldsymbol{y}_1^T - \boldsymbol{y}_1\boldsymbol{y}_2^T\right) \\
                & = \boldsymbol{I} + j\left[
                    \begin{array}{cc}
                        0 & -\eta \\
                        \eta &  0
                    \end{array}
                \right], 
            \end{align}
        \end{subequations}
        where $\eta = y_{11}y_{22} - y_{12}y_{21} = \text{det}(\boldsymbol{Y}) = \pm 1$ because $\boldsymbol{Y}$ is an orthogonal matrix. 
        If $\text{det}(\boldsymbol{Y}) = 1$, we have 
        \begin{equation}
            \boldsymbol{J} = \left[
                \begin{array}{cc}
                    1 & -j \\
                    j &  1
                \end{array}
            \right], \ \hat{\boldsymbol{H}} = \left[
                    \begin{array}{c}
                        \bar{\boldsymbol{A}} \\
                        \bar{\boldsymbol{B}}
                    \end{array}
                \right]\boldsymbol{J}\left[
                    \bar{\boldsymbol{A}}^T, \bar{\boldsymbol{B}}^T
                \right] = \bar{\boldsymbol{H}}. 
        \end{equation}
        If $\text{det}(\boldsymbol{Y}) = -1$, however, $\boldsymbol{J}$ and $\hat{\boldsymbol{H}}$ are given as 
        \begin{equation}
            \boldsymbol{J} = \left[
                \begin{array}{cc}
                    1 & j \\
                    -j &  1
                \end{array}
            \right], \ \hat{\boldsymbol{H}} = \left[
                    \begin{array}{c}
                        \bar{\boldsymbol{A}} \\
                        \bar{\boldsymbol{B}}
                    \end{array}
                \right]\boldsymbol{J}\left[
                    \bar{\boldsymbol{A}}^T, \bar{\boldsymbol{B}}^T
                \right] = \bar{\boldsymbol{H}}^*. 
        \end{equation}
        Hence, $\bar{\boldsymbol{H}}$ and $\bar{\boldsymbol{H}}^*$ are the only two solutions to Problem~\eqref{prob:cov-est-find-origin} with probability $1$ when $b = 1$, $N\ge 6$ and $T_{p}$ is sufficiently large. 
        Hereto, the proof for the existence and uniqueness of the solutions to Problem~\eqref{prob:cov-est-find-origin} claimed in Proposition~\ref{prop:cov-est-existence-uniqueness} have been completed. 


